Refiner: Restructure Retrieval Content Efficiently to Advance Question-Answering Capabilities

Large Language Models (LLMs) are limited by their parametric knowledge, leading to hallucinations in knowledge-extensive tasks. To address this, Retrieval-Augmented Generation (RAG) incorporates external document chunks to expand LLM knowledge. Furthermore, compressing information from document chunks through extraction or summarization can improve LLM performance. Nonetheless, LLMs still struggle to notice and utilize scattered key information, a problem known as the "lost-in-the-middle" syndrome. Therefore, we typically need to restructure the content for LLM to recognize the key information. We propose $\textit{Refiner}$, an end-to-end extract-and-restructure paradigm that operates in the post-retrieval process of RAG. $\textit{Refiner}$ leverages a single decoder-only LLM to adaptively extract query-relevant contents verbatim along with the necessary context, and section them based on their interconnectedness, thereby highlights information distinction, and aligns downstream LLMs with the original context effectively. Experiments show that a trained $\textit{Refiner}$ (with 7B parameters) exhibits significant gain to downstream LLM in improving answer accuracy, and outperforms other state-of-the-art advanced RAG and concurrent compressing approaches in various single-hop and multi-hop QA tasks. Notably, $\textit{Refiner}$ achieves a 80.5% tokens reduction and a 1.6-7.0% improvement margin in multi-hop tasks compared to the next best solution. $\textit{Refiner}$ is a plug-and-play solution that can be seamlessly integrated with RAG systems, facilitating its application across diverse open-source frameworks.

==> table/refiner_output_example.tex <==
\begin{table*}[ht!]
\caption{Case study of how compressing the retrieved documents helps the model to identify the right answer from NQ dev set.}
\scriptsize
\begin{tabular}{p{2cm}p{9cm}p{3cm}}
\toprule
\multicolumn{2}{l}{\textit{Question: host of the late show who was once a correspondent for the daily show.}} &  \textit{Gold answer: Stephen Colbert} \\
\toprule
\textbf{Type} & \textbf{In-context documents} & \textbf{Predicted Answers} \\ 
\midrule
None &  & Chelsea Handler	 \\ \hline
Top 5 & by Conan O\'Brien, in 2009. Leno explained that he did not want to see a repeat of the hard feelings and controversy that occurred when he was given the show over David Letterman following Carson\'s retirement in 1992. O\'Brien\'s last "Late Night" episode was taped on February 20, 2009. Former Saturday Night Live alum Jimmy Fallon took over as host of "Late Night with Jimmy Fallon" on March 2, 2009. The Colbert Report that aired four days a week on Comedy Central from October 17, 2005, was hosted by Stephen Colbert, one of the regulars on Comedy Central\'s The Daily
season as host began with a notable interview with former British prime minister Tony Blair. The live interview occurred the night before a book signing at Eason's which attracted international attention when Blair was pelted with shoes and eggs and successfully evaded an attempted citizen's arrest on charges of war crimes. On 1 February 2013, Pat Kenny returned to host that night's edition when Tubridy's father died. In 2015, Tubridy's tone and choice of questions when interviewing Anti-Austerity Alliance TD Paul Murphy in relation to the campaign against the implementation of a water tax was much criticised. Opponents of the
'Michigan, interviewing Eminem. Colbert has been given near-full control of the show, with little interference from CBS management in regard to format. Colbert brought most of his staff from "The Colbert Report" with him to "The Late Show", as well as outsiders such as Brian Stack, who is best known for his work on Conan O\'Brien\'s programs, and Jon Stewart, former host of Colbert\'s previous sister program "The Daily Show", who is credited as executive producer. Colbert no longer uses the character he had portrayed on "The Colbert Report", jokingly remarking to Jeb Bush that "I used to play a 
Show" has had three regular hosts: Gay Byrne, Pat Kenny and Ryan Tubridy. Frank Hall deputised for Byrne for one season in the 1960s. There have been at least four occasions on which another presenter has hosted the show. The first was when Byrne became unexpectedly and seriously ill. Frequent panelist Ted Bonner presented instead. The second time was towards the end of a show about feminism, when Byrne ushered a young Marian Finucane into his seat to present the remainder of the show. On another occasion, radio broadcaster and former news reader Andy O\'Mahony replaced Byrne for an interview
popular acclaim. Colbert would host the program until he was chosen to replace David Letterman as host of CBS\'s "Late Show" in 2015. Ed Helms, a former correspondent from 2002 to 2006, also starred on NBC\'s "The Office" and was a main character in the 2009 hit "The Hangover". After filling in as host during Stewart\'s two-month absence in the summer of 2013, John Oliver went on to host his own show on HBO, "Last Week Tonight with John Oliver". In 2016, former correspondent Samantha Bee launched her own late-night talk show "Full Frontal with Samantha Bee". Bee\'s husband Jason & Samantha Bee \\ 
\midrule 
GPT-3.5-turbo & Former Daily Show correspondent Stephen Colbert was chosen to replace David Letterman as host of CBS's "Late Show" in 2015, while Ed Helms, a former correspondent from 2002 to 2006, also starred on NBC's "The Office" and John Oliver, who filled in as host during Jon Stewart's absence in 2013, went on to host his own show on HBO. \\ \midrule
T5 (ours) & Stephen Colbert was a former correspondent for The Daily Show and later became host of CBS's "Late Show" in 2015. He has since brought most of his staff from "The Colbert Report" with him to "The Late Show", with little interference from CBS management in regard to format. & Stephen Colbert \\
\bottomrule
\end{tabular} \vspace{-0.3em}
\label{tab:case_study}
\end{table*}

